Principal-Agent Problem with Third Party: Information Design from Social Planner's Perspective

We study the principal-agent problem with a third party that we call social planner, whose responsibility is to reconcile the conflicts of interest between the two players and induce socially optimal outcome in terms of some given social utility function. The social planner owns no contractual power but manages to control the information flow between the principal and the agent. We design a simple workflow with two stages for the social planner. In the first stage, the problem is reformulated as an optimization problem whose solution is the optimal utility profile. In the second stage, we investigate information design and show that binary-signal information structure suffices to induce the socially optimal outcome determined in the first stage. The simplicity and modularity of our method make it easy to implement in various scenarios within the principal-agent problem.

==> appenbp.tex <==
There are several fundamental differences between information design in the principal-agent problem and the seminal work of Bayesian persuasion~\citep{kamenica2011bayesian}.

In Bayesian persuasion, the model consists of two players, a sender and a receiver, where the sender is the information structure (signaling scheme) designer. Owing to the superiority of knowing the realized state of nature, the sender designs the signaling scheme such that the receiver would take an action maximizing the sender's payoff, where the model assumes that the sender and the receiver shares a common prior distribution over the states of nature. In the information design in principal-agent problem, there are three players, the social planner, the principal and the agent, where the social planner designs the information structure, the principal then designs a contract based on the information structure and finally the agent takes the action which maximizes her own utility function and affects the payoff of both the principal and the society. In Bayesian persuasion, the signaling scheme is designed for each possible state of nature, while in principal-agent problem, the information structure is depicted for each available actions for the agent. A fundamental difference between these two scenarios is that the Bayesian persuasion sender is merely an observer and has no power to change the state of nature, while in the principal-agent model, different information structures induce different contract designed by the principal, and would in turns induce different optimal actions for the agent. Therefore, in some sense, the information design problem is more complicated than Bayesian persuasion.

However, in another sense, the information structure is simpler in the principal-agent model than in the Bayesian persuasion model. As is noted in \citet[Proposition 1]{kamenica2011bayesian}, the signaling scheme in Bayesian persuasion has a close relationship to the revelation principle~\citep{myerson1979incentive}, i.e., the sender only needs to design signaling scheme that directly recommends actions to the receiver. Therefore, in the basic model of Bayesian persuasion, researchers usually assume that the signal space is not smaller than the state space and the action space~\citep{kamenica2019bayesian}, i.e., $\abs{S} \geq \min \left\{\abs{\Omega}, \abs{A}\right\}$. This would raise an issue if the state space and the action space are both large while the availability of messages is limited, \citet{aybas2019persuasion} shows that the sender's utility would always be worse off with coarse communication. Fortunately, in the information design in principal-agent problem, such difficulty need hardly be taken into account. Although there are infinite available contracts for the principal and $n$ possible actions for the agent, the social planner needs only care about binary-signal information structure. Such ``blessing'' comes from the specific structure of the principal-agent problem. The agent's utility function consists of two parts, i.e., the cost for the chosen action and the expected monetary transfer. Therefore, if two actions share the same expected transfer, the one with cheaper cost always dominates, and hence we can simply divide the actions into two groups: one group employs the socially optimal action $a^*$, i.e., the corresponding action for the optimal utility profile that the social planner would like to induce, as the dominated action, while the other group employs action $\hat{a}$, which by definition is the action with the maximum expected reward for the principal among all the least costly actions for the agent, as the dominant. From this observation, it suffices for the principal to design a contract with binary-choice monetary transfer, since the size of the ``state space'' is two.


==> appenpa.tex <==
In economic theory, the principal-agent problem typically arises where the two parties have different interests and asymmetric information. Concerning the information asymmetry, the model can be divided into two categories: (a) moral hazard~\citep{holmstrom1979moral} where the actions of the agent is not observed and (b) adverse selection~\citep{hart1987theory} where the characteristics of the agent is not observed. 

The setting considered in this paper is closely related to the moral hazard model, where the agent takes some actions which the principal cannot observe, but instead some signals from those actions are revealed and contracts should be written on those signals.
However, there are two main differences. 
First, in classic principal-agent model, the signal not only provides the principal with some information about the agent's action, but also specifies the profit or reward for the principal, while the information structure in our model has no role in determining the income for the principal. 
Second, classic principal-agent model involves two parties and mainly focus on designing the optimal contract from the principal's point of view, assuming that the agent is rational.
In this work, we introduce a third party, the social planner, who acts as a conciliator between the principal and the agent. By controlling the information flow, the social planner has great power to decide ``where the game is going''. The main purpose of our work is to design the information structure toward a specific social purpose characterized by a social utility function, assuming that both the principal and the agent are rational that each of them would maximize their own utility function. The workflow proposed in this work provides insight for the minimum amount of information needed to induce certain equilibrium of the system. 
Whether the information design process developed in this work can be extended to the model of adverse selection problem, i.e., the system is not fully known to the social planner while the principal and/or the agent may be informed some private messages before the information structure is designed, would be an interesting future direction.

